Hate Speech Detection in Limited Data Contexts using Synthetic Data Generation

A growing body of work has focused on text classification methods for detecting the increasing amount of hate speech posted online. This progress has been limited to only a select number of highly-resourced languages causing detection systems to either under-perform or not exist in limited data contexts. This is majorly caused by a lack of training data which is expensive to collect and curate in these settings. In this work, we propose a data augmentation approach that addresses the problem of lack of data for online hate speech detection in limited data contexts using synthetic data generation techniques. Given a handful of hate speech examples in a high-resource language such as English, we present three methods to synthesize new examples of hate speech data in a target language that retains the hate sentiment in the original examples but transfers the hate targets. We apply our approach to generate training data for hate speech classification tasks in Hindi and Vietnamese. Our findings show that a model trained on synthetic data performs comparably to, and in some cases outperforms, a model trained only on the samples available in the target domain. This method can be adopted to bootstrap hate speech detection models from scratch in limited data contexts. As the growth of social media within these contexts continues to outstrip response efforts, this work furthers our capacities for detection, understanding, and response to hate speech.

==> Sections/results.tex <==
Figure \ref{fig:accuracy_norm} shows the results of experiments when no hateful posts are available in the low resource language and we synthetically have to generate all the hateful posts. We evaluate the performance our trained models on both the test set distributions.

Through our experiments, we find that the mBERT model fine-tuned on the \textit{Synthetic-IS} dataset almost always outperforms the other two synthetic data generation strategies. In figure \ref{fig:vis1} the performance of the model decreases as we increase the size of the synthetically generated hateful posts since the synthetic data starts adding noise but here we find that the \textit{Synthetic-IS} augmentation strategy adds lesser noise to the training as compared to the vanilla translation strategy or the synthetic data generation strategy with replacement.

In figure \ref{fig:vis3}, however, we observe that when evaluated on the diversified test set, the performance of the model fine-tuned on the \textit{Synthetic-IS} data comes very close to the performance of the model trained on \textit{Original} dataset. This, we believe, strongly reflects the strength of our synthetic data generation strategy since we often encounter settings similar to the diversified testing setting when we deploy hate-speech detection models on the field in low-resource settings.
% We were also able to bridge the gap between a model fine-tuned on original data taken from the low-resource language and a model fine-tuned on the synthetically generated data.

Next, table \ref{tab:accuracy_aug} shows the average accuracy and F1 score of our data augmentation experiments with our evaluations being done on the diversified test set distribution since it more closely resembles our on-field experience.

\begin{table}[b]
  \centering
  \caption{Average accuracy of models trained after augmenting 50 original hate-speech posts and 1000 non-hateful posts}
  \label{tab:accuracy_aug}
  \begin{tabular}{c|c|c}
    Data Type & Accuracy & F1 \\
    \hline
    No-Augmentation & 51.70 & 0.00 \\
    Translated & 51.01 & 0.00 \\
    Synthetic & 52.15 & 0.00 \\
    Synthetic-IS & \textbf{52.27} & 0.00
    % & & Unexplained usage\\
  \end{tabular}
\end{table}

The key takeaways from this experiment are that the mBERT model fine-tuned on augmented datasets outperform the models trained on a dataset without any augmentation i.e. just a dataset comprising of an extremely imbalanced data. When we augment the original 50 hate-speech posts with a vanilla translation of the English hate-speech posts, we find that the accuracy rather drops which means the translation adds more noise to the data rather than adding any value. Augmentation with the synthetic datasets however adds more value to the performance of the model.


% \begin{figure}[t]
%      \centering
%      \begin{subfigure}[b]{0.5\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Plots/paper_plot_1.png}
%          \caption{Original test set}
%          \label{fig:orig_test_set_norm}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.5\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Plots/paper_plot_3.png}
%          \caption{Diversified test set}
%          \label{fig:div_test_set}
%      \end{subfigure}
%      \hfill
%         \caption{Accuracy plots}
%         \label{fig:Accuracy plots}
% \end{figure}

% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.5\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Plots/paper_plot_1.png}
%          \caption{Original test set}
%          \label{fig:orig_test_set_norm}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.5\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Plots/paper_plot_3.png}
%          \caption{Diversified test set}
%          \label{fig:div_test_set}
%      \end{subfigure}
%      \hfill
%         \caption{Accuracy plots}
%         \label{fig:Accuracy plots}
% \end{figure}

